Studying the Impact of Early Test Termination Due to Assertion Failure on Code Coverage and Spectrum-based Fault Localization

An assertion is commonly used to validate the expected programs behavior (e.g., if the returned value of a method equals an expected value) in software testing. Although it is a recommended practice to use only one assertion in a single test to avoid code smells (e.g., Assertion Roulette), it is common to have multiple assertions in a single test. One issue with tests that have multiple assertions is that when the test fails at an early assertion (not the last one), the test will terminate at that point, and the remaining testing code will not be executed. This, in turn, can potentially reduce the code coverage and the performance of techniques that rely on code coverage information (e.g., spectrum-based fault localization). We refer to such a scenario as early test termination. Understanding the impact of early test termination on test coverage is important for software testing and debugging, particularly for the techniques that rely on coverage information obtained from the testing. We conducted the first empirical study on early test termination due to assertion failure (i.e., early test termination) by investigating 207 versions of 6 open-source projects. We found that a nonnegligible portion of the failed tests (19.1%) is early terminated due to assertion failure. Our findings indicate that early test termination harms both code coverage and the effectiveness of spectrum-based fault localization. For instance, after eliminating early test termination, the line/branch coverage is improved in 55% of the studied versions, and improves the performance of two popular SBFL techniques Ochiai and Tarantula by 15.1% and 10.7% compared to the original setting (without eliminating early test termination) in terms of MFR, respectively.

==> datapreparation.tex <==
\section{Data Preparation}\label{sec:datapreparation}



==> rq4.tex <==
\subsection*{\rqfour}\label{sec:rq4}


\textbf{\slicing outperforms or has the same performance as \trycatch for SBFL (both Ochiai and Tarantula) in terms of MFR and EXAM in all projects. For Ochiai, \slicing improves \trycatch by 9.8\% and 4.1\% in terms of MFR and EXAM, respectively.}
\slicing outperforms or has the same performance as \trycatch in terms of EXAM and MFR in all studied projects as shown Table~\ref{tab:FLresults}. On average, for Ochiai, \slicing improves \trycatch by 9.8\% and 4.1\% in terms of MFR and EXAM, respectively. Let's consider the two largest projects math and lang. In math, \slicing improves MFR and EXAM scores both by 21.6\% and 2.6\% for Ochiai compared with \trycatch, respectively. In lang, \slicing improves MFR and EXAM by 13.1\%, 3.4\% for Ochiai, respectively. In terms of Top@k, for Ochiai, in lang, we observe that \slicing outperforms \trycatch by 54.9\% and 45.7\% when k equals 5 and 10, respectively. In other relatively smaller projects, \slicing has better or equivalent performance as \trycatch. We observe a similar trend for Tarantula. If we compare \slicing with \original, the improvement is even more remarkable. For instance, on average, for Ochiai, \slicing improves \original by 15.1\% and 4.4\% in terms of MFR and EXAM, respectively.




%If we look at the largest two projects math and lang. In math, \slicing improves MFR and EXAM by 21.6\%, 2.6\% respectively, compared with \trycatch. In lang, \slicing improves MFR and EXAM by 13.1\%, 3.4\%, respectively, compared with \trycatch. In terms of Top@k, in lang, we observe that \slicing outperforms \trycatch by 54.9\% and 45.7\% when k equals 5 and 10, respectively. While in math, \trycatch performs better than \slicing. In other relatively smaller projects, \slicing has better or equivalent performance as \trycatch.

%\textbf{\slicing improves the performance of SBFL in 30\% of the studied versions, while \trycatch only improves in 18.3\% of the versions.} To better understand in which cases the performance gets improved and deteriorated. We present Table~\ref{tab:FL_versionwise} to show the number of versions in which the performance of Ochiai gets tied, improved, and deteriorated after applying \slicing and \trycatch. We observe that in the majority of the versions, the performance of SBFL gets tied. This is reasonable, since as Table~\ref{tab:RQ2_versionwise} shows, in around 45\% (27 out of 60) of the versions, the line coverage does not change after applying \slicing and \trycatch. Across all projects, we observe that \slicing and \trycatch improve the performance of Ochiai in 30\% (18 out of 60) and 18.3\% (11 out of 60), respectively. Overall, \slicing outperforms \trycatch. %, which is as expected.
%We illustrate why \slicing outperforms \trycatch using an example.

\begin{table}[]
\scriptsize
\caption{The number of versions that get improved (Imp), deteriorated (Det), and tied after applying Trycatch and Slicing compared with original for Ochiai (first value in each cell) and Tarantula (second value) in terms
of MFR, respectively.}
\label{tab:FL_versionwise}


\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|rrr|rrr}
\hline
     & \multicolumn{3}{c|}{\textbf{Original vs Trycatch}}    & \multicolumn{3}{c}{\textbf{Trycatch vs Slicing}}    \\
\hline
\textbf{Project} & \textbf{\#Tied} & \textbf{\#Imp} & \textbf{\#Det} & \textbf{\#Tied} & \textbf{\#Imp}  &\textbf{\#Det} \\
\hline
math     & 23/23 & 3/3 & 3/3 & 22/23 & 4/4 & 3/2 \\
joda-time  & 3/3 & 1/1 & 1/1 & 0/0 & 5/5 & 0/0 \\
jfreechart  & 1/2 & 0/0 & 1/0 & 2/2 & 0/0 & 0/0 \\
jackson-core & 1/1 & 1/1 & 0/0 & 1/2 & 1/0 & 0/0 \\
fastjson   & 0/0 & 3/4 & 1/0 & 0/1 & 1/2 & 3/1 \\
lang     & 12/12 & 3/3 & 3/3 & 10/8 & 6/7 & 2/3 \\
\hline
\textbf{Total}    & 35/36 & 11/12 & 9/7 & 37/34 & 17/18 & 8/6 \\
\hline
\end{tabular}
}

%\resizebox{0.7\textwidth}{!}{
%\begin{tabular}{l|lll|lll}
%\hline
 %    & \multicolumn{3}{c|}{\textbf{Original vs Slicing (Ochiai)}}    & \multicolumn{3}{c}{\textbf{Original vs Slicing (Tarantula)}}    \\
%\hline
%\textbf{Project} & \textbf{\#Tied} & \textbf{\#Imp} & \textbf{\#Det} & \textbf{\#Tied} & \textbf{\#Imp} & \textbf{\#Det} \\
%\hline
%math     & 23 & 5 & 1 & 23 & 5 & 1 \\
%joda-time  &  0  & 5 & 0 &  0  & 5 & 0 \\
%jfreechart  & 1  & 0 & 1 & 2  & 0 & 0 \\
%jackson-core & 1  & 1 & 0 & 1  & 1 & 0 \\
%fastjson   & 0  & 3 & 1  &0  & 4 & 0 \\
%lang     & 12 & 4 & 2 & 8 & 7 & 3 \\
%\hline
%\textbf{Total}    & 37 & 18 & 5 & 34 & 22 & 4 \\
%\hline
%\end{tabular}
%}
\vspace{-0.1in}
\end{table}
\noindent\textbf{\slicing improves the performance of SBFL in 28.3\% and 30\% studied versions over \trycatch for Ochiai and Tarantula, respectively.}
We present the comparison between \slicing and \trycatch in  Tables~\ref{tab:FL_versionwise}. We observe that \slicing outperforms \trycatch in 17 and 18 out of 60 versions for Ochiai and Tarantula, respectively. Overall, \slicing outperforms \trycatch in terms of both SBFL.


%\sw{Ahsraf: need a case to show why \slicing outperform \trycatch}
Now let us use an example to illustrate why \slicing outperforms \trycatch. For instance, in version 41 of the project lang, there are 1,624 runnable tests after applying \trycatch. Among those tests, there are two failed tests. However, after applying \slicing, the number of total runnable tests is increased to 1661, with a total of 17 failures among them, which indicates there are 15 more failed tests. In this case, the buggy lines are only executed in two failed tests when applying \trycatch, while are executed in 17 failed tests when applying \slicing. When the number of those failed tests is plugged into the Ochiai and Tarantula formulas, we get the rank of the first buggy line for \trycatch and \slicing at 7 and 3 for Ochiai, and at 8 and 5 for Tarantula. \slicing alleviates the limitation of \trycatch (i.e., aggregating all assertion failures in a test into a single testing result) and provides a finer-grained test result.

\rqboxc{Overall, \slicing outperforms \trycatch for SBFL. For instance, \slicing improves \trycatch by 9.8\% and 4.1\% in terms of MFR and EXAM for Ochiai, respectively. \slicing improves the performance of SBFL in 28.3\% of the studied version over \trycatch.}


\begin{comment}
\ashraf{In some cases, when tests are run few statements are partially covered while applying \trycatch and \slicing techniques, and those statements are not missed by the code coverage report. After analyzing Cyclomatic Complexity we found that in some cases, \trycatch partially covers a few conditional statements while \slicing fully covers those statements. For instance, in the case of joda-time version 8, we get the MFR for \trycatch and \slicing 162 and 149 respectively for Ochiai, and 167 and 118 for Tarantula while applying \trycatch and \slicing respectively. When \trycatch is applied, line number 135 is partially covered which is shown in Figure \ref{fig:trycatch}. However, upon implementing \slicing line number 135 is fully covered and it is shown in Figure \ref{fig:slicing}. As a result, \slicing outperforms \trycatch in some versions.} 

\begin{figure}
    \centering

\includegraphics [width=\textwidth, height=0.6\linewidth]{figures/trycatch.png}
    \caption {An example after applying Trycatch}
    \label{fig:trycatch}
    
\end{figure}

\begin{figure}
    \centering

\includegraphics[width=\textwidth, height=0.6\linewidth]{figures/slicing.png}
    \caption {An example after applying Slicing}
    \label{fig:slicing}
    
\end{figure}
  


\end{comment}








